Development of large scale CVD grown two dimensional materials for field-effect transistors, thermally-driven neuromorphic memory, and spintronics applications

Semiconductor research has shifted towards exploring two-dimensional (2D) materials as candidates for next-generation electronic devices due to the limitations of existing silicon technology. Transition Metal Dichalcogenides (TMDCs) stand out for their exceptional optoelectronic properties and potential for advanced device integration. This thesis focuses on the synthesis of 2D TMDCs using Chemical Vapor Deposition (CVD) for their potential applications in transistors, memory, and neuromorphic computing. By optimizing the NaCl-assisted CVD method and examining their optical properties through Raman and photoluminescence spectroscopy, challenges such as premature growth, defects, and non-uniformity in MoS2 samples are addressed. The thesis highlights device fabrication techniques and electrical performance of salt-assisted CVD-grown MoS2 field-effect transistors, which exhibit hysteresis-free behavior and high field-effect mobility. A novel etching-free transfer technique is introduced, improving transistor performance and enabling applications in flexible optoelectronics. The thesis also explores monolayer MoS2 mem-transistors, demonstrating multifunctional room temperature transistor and high-temperature multi-level memory behaviour. These devices leverage interfacial physics and ion dynamics to achieve non-volatile memory with multi-level storage capabilities. Additionally, high density memory devices using monolayer WS2 are developed, which demonstrate 6-bit memory operation with neuromorphic biomimetic plasticity. The study also includes 2D TMDCs and their hetero-bilayers as potential 2D dilute magnetic semiconductors via doping, strain engineering using density functional theory and micromagnetic simulations, revealing potential applications in spintronics. This thesis makes significant contributions to advancing 2D materials for next-generation electronics and spintronic devices.

==> chapters/backup.tex <==
\begin{align}
{\cal E}_{{\rm NM}} & = \sum_{\alpha=p,n} \frac{1}{\pi^2}\int_{0}^{k_{\alpha}} k^2\, dk \, {\cal{E}_\alpha^*} +\rho_b\,g_\omega\,\omega-\frac{1}{4!}\zeta_{0}\,{g_{\omega}^2}\,\omega^4+ \frac{1}{2}\rho_{b3}\,g_\rho\,\rho 
\nonumber\\
&
+m_{\sigma}^2{\sigma}^2\left(\frac{1}{2}+\frac{\kappa_{3}}{3!}\frac{g_\sigma\sigma}{M}+\frac{\kappa_4}{4!}\frac{g_\sigma^2\sigma^2}{M^2}\right)-\frac{1}{2}m_{\omega}^2\,\omega^2\left(1+\eta_{1}\frac{g_\sigma\sigma}{M}+\frac{\eta_{2}}{2}\frac{g_\sigma^2\sigma^2}{M^2}\right) \nonumber\\
& 
- \frac{1}{2}\left(1+\frac{\eta_{\rho}g_\sigma\sigma}{M}\right)m_{\rho}^2\,\rho^{2}
+\frac{1}{2}m_{\delta}^2\, \delta^{2},
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{align}
P_{{\rm NM}} & = \sum_{\alpha=p,n} \frac{1}{3\pi^2}\int_{0}^{k_{\alpha}} dk\,  \frac{k^4}{{\cal E}_\alpha^\ast} + \frac{1}{4!}\zeta_{0}\,{g_{\omega}^2}\,\omega^4 +\Lambda_{\omega}\, g_\rho^2\, g_\omega^2\, \rho^2\, \omega^2
\nonumber\\
&
- m_{\sigma}^2{\sigma}^2\left(\frac{1}{2} + \frac{\kappa_{3}}{3!}\frac{g_\sigma\sigma}{M} + \frac{\kappa_4}{4!}\frac{g_\sigma^2\sigma^2}{M^2}\right)+\frac{1}{2}m_{\omega}^2\,\omega^2\left(1+\eta_{1}\frac{g_\sigma\sigma}{M}+\frac{\eta_{2}}{2}\frac{g_\sigma^2\sigma^2}{M^2}\right)
\nonumber\\
&
+ \frac{1}{2}\left(1+\frac{\eta_{\rho}g_\sigma\sigma}{M}\right)m_{\rho}^2\,\rho^{2}-\frac{1}{2}m_{\delta}^2\, \delta^{2}.
\end{align}


%%%%%%%%%%%%%
\begin{align}
{\cal E}({r})&=\sum_{\alpha=p,n} \varphi_\alpha^\dagger({r})\Bigg\{-i \mbox{\boldmath$\alpha$} \!\cdot\!\mbox{\boldmath$\nabla$}+\beta \left[M_\alpha-\Phi (r)-\tau_3 D(r)\right] +W({r})+\frac{1}{2}\tau_3 R({r})
\nonumber\\
&
+\frac{1+\tau_3}{2}A({r})-\frac{i\beta\mbox{\boldmath$\alpha$}}{2M}\!\cdot\!\left(f_\omega\mbox{\boldmath$\nabla$}W({r})+\frac{1}{2}f_\rho\tau_3 \mbox{\boldmath$\nabla$}R({r})\right)\Bigg\} \varphi_\alpha(r)
\nonumber\\
&
-\frac{\zeta_0}{4!}\frac{1}{g_\omega^2}W^4({r})+\left(\frac{1}{2}+\frac{\kappa_3}{3!}\frac{\Phi({r})}{M}+\frac{\kappa_4}{4!}\frac{\Phi^2({r})}{M^2}\right)\frac{m_s^2}{g_\omega^2}\Phi^2({r})
\nonumber\\
&
+\frac{1}{2g_\sigma^2}\times\left(1+\alpha_1\frac{\Phi({r})}{M}\right)\left(
\mbox{\boldmath $\nabla$}\Phi({r})\right)^2-\frac{1}{2g_\omega^2}
\left( 1+\alpha_2\frac{\Phi({r})}{M}\right)\left(\mbox{\boldmath$\nabla$} W({r})\right)^2
\nonumber\\
&
-\frac{1}{2}\left(1+\eta_1\frac{\Phi({r})}{M}+\frac{\eta_2}{2} \frac{\Phi^2({r})}{M^2}\right)\frac{m_\omega^2}{g_\omega^2} W^2({r})-\frac{1}{2e^2} \left( \mbox{\boldmath $\nabla$} A({r})\right)^2-\frac{1}{2g_\rho^2} \left( \mbox{\boldmath $\nabla$} R({r})\right)^2
\nonumber\\
&
-\frac{1}{2} \left( 1 + \eta_\rho \frac{\Phi({r})}{M}\right)\frac{m_\rho^2}{g_\rho^2} R^2({r})-\Lambda_{\omega}\left(R^{2}(r)\times W^{2}(r)\right)
\nonumber\\
& 
 +\frac{1}{2 g_{\delta}^{2}}\left(\mbox{\boldmath $\nabla$} D({r})\right)^2+\frac{1}{2}\frac{{m_{\delta}}^2}{g_{\delta}^{2}}D^{2}(r)\;,
\label{eq:rmf_edf}
\end{align}
%%%%%%%%%%%%%%
where $\Phi$, $W$, $R$, $D$, and $A$ are the fields with $\Phi=g_{\sigma}\sigma, W=g_{\omega} \omega, R=g_{\rho} \rho, {\rm and}\ D=g_{\delta}\delta$ respectively; $g_\sigma$, $g_\omega$, $g_\rho$, $g_\delta$ are the coupling constants; and $m_\sigma$, $m_\omega$, $m_\rho$, and $m_\delta$ are the masses for $\sigma$, $\omega$, $\rho$, and $\delta$ mesons respectively. The parameters, such as $\eta_{1}, \eta_{2}, \Lambda_{\omega}, \alpha_{1}, \alpha_{2}, f_{\omega}$, and $f_\rho$ are the different cross coupling terms. The term $\frac{e^2}{4\pi}$ is the photon coupling constant. $M_\alpha$ represent the masses of nucleons.

The single-particle energy for the nucleons is obtained by using the Lagrange multiplier $\varepsilon_\alpha$, which is the energy eigenvalue of the Dirac equation constraining the normalization condition $\sum_\alpha\varphi_\alpha^\dagger({r}) \varphi_\alpha({r})=1$.  
The Dirac equation for the wave function $\varphi_\alpha({r})$ becomes
%%%%%%%%%%%%%%%%
\begin{align}
\frac{\partial}{\partial\varphi_\alpha^\dagger({r})}\Bigg[{\cal E}{({r})}-
\sum_\alpha\varphi_\alpha^\dagger({r}) \varphi_\alpha({r})\Bigg]= 0,
\label{eq:nucleon_minima}
\end{align}
%%%%%%%%%%%%%%%%
which implies that 
%%%%%%%%%%%%%
\begin{align}
\Bigg\{-i \mbox{\boldmath$\alpha$} \!\cdot\! \mbox{\boldmath$\nabla$} \, 
+\beta [M - \Phi(r) - \tau_3 D(r)] + W(r)+\frac{1}{2} \tau_3 R(r) + \frac{1 +\tau_3}{2}A(r)
\nonumber\\
\left.
-\frac{i\beta \mbox{\boldmath$\alpha$}}{2M}\!\cdot\! \left [f_\omega \mbox{\boldmath$\nabla$} W(r)+\frac{1}{2}f_{\rho} \tau_3 \mbox{\boldmath$\nabla$} R(r) \right]
\right\} \varphi_\alpha (r) =
\varepsilon_\alpha \, \varphi_\alpha (r) \,.
\label{eq:nucleon_wavefn}
\end{align}
%%%%%%%%%%%
The mean-field equations for $\Phi$, $W$, $R$, $D$, and $A$ are given by
%%%%%%%%%%%%%
\begin{align}
-\Delta \Phi(r) + m_\sigma^2 \Phi(r) &= g_\sigma^2 \rho_s(r)-{m_\sigma^2\over M}\Phi^2 (r)\left({\kappa_3\over 2}+{\kappa_4\over 3!}{\Phi(r)\over M}\right)
\nonumber \\
&
+{g_\sigma^2 \over 2M}\left(\eta_1+\eta_2{\Phi(r)\over M}\right){m_\omega^2\over g_\omega^2} W^2 (r)+{\eta_{\rho} \over 2M}{g_\sigma^2 \over g_\rho^2}{m_\rho^2 } R^2 (r)
\nonumber\\
&
+{\alpha_1 \over 2M}\left[(\mbox{\boldmath $\nabla$}\Phi(r))^2+2\Phi(r)\Delta \Phi(r)\right]
+{\alpha_2 \over 2M} {g_s^2\over g_\omega^2}\left(\mbox{\boldmath $\nabla$}W(r)\right)^2, 
\label{eq:sigma_field}
\end{align}
%%%%%%%%%%%%%
\begin{align}
-\Delta W(r)+m_\omega^2 W(r)&=g_\omega^2 \left(\rho_b(r)+\frac{f_\omega}{2} \rho_{\rm T}(r) \right)-\left( \eta_1+{\eta_2\over 2}{\Phi(r)\over M} \right){\Phi(r)\over M} m_\omega^2 W(r)
\nonumber\\
&
-{1\over 3!}\zeta_0 W^3(r)+{\alpha_2 \over M} [\mbox{\boldmath $\nabla$}\Phi(r) \cdot\mbox{\boldmath $\nabla$}W(r)+\Phi(r)\Delta W(r)]
\nonumber\\
&
-2\;\Lambda_{\omega}{g_{\omega}}^2 {R^{2}(r)} W(r) \,,
\label{eq:omega_field}
\end{align}
%%%%%%%%%%%%%%%%
\begin{align}
-\Delta R(r)+ m_{\rho}^2 R(r)&={1 \over 2 }g_{\rho}^2 \left (\rho_{b3}(r) +
{1 \over 2 }f_{\rho}\rho_{\rm T,3}(r)\right ) - \eta_\rho {\Phi (r) \over M }m_{\rho}^2 R(r)
\nonumber\\
&
-2\;\Lambda_{\omega}{g_{\rho}}^{2} R(r) {W^{2}(r)} \,,
\label{eq:rho_field}
\end{align}
%%%%%%%%%%%%%%%%
\begin{align}
-\Delta D(r)+{m_{\delta}}^{2} D(r) = g_{\delta}^{2}\rho_{s3} \, ,
\label{eq:delta_field}
\end{align}
%%%%%%%%%%%%%%%%
\begin{align}
-\Delta A(r)=e^2 \rho_{\rm p}(r) \,, 
\label{eq:photon_field}
\end{align}
%%%%%%%%%%%%%%%%
where the baryon, scalar, isovector, proton, and tensor densities are
%%%%%%%%%%%%
\begin{align}
\rho_b(r) = \sum_{\alpha=p,n} \left\langle \varphi_\alpha^\dagger(r) \varphi_\alpha(r) \right\rangle\,
=\rho_{p}(r)+\rho_{n}(r)
=\sum_{\alpha=p,n}\frac{1}{\pi^2}\int_{0}^{k_\alpha}k^2 dk \, ,
\label{eq:baryon_density} 
\end{align}
%%%%%%%%%%%%
\begin{align}
\rho_s(r)=\sum_{\alpha=p,n} \left\langle \varphi_\alpha^\dagger(r) \beta \varphi_\alpha(r)\right\rangle
=\rho_{s p}(r)+\rho_{s n}(r)
=\sum_{\alpha=p,n} \frac{M_\alpha^{\ast}}{\pi^2}\int_{0}^{k_\alpha} dk \, \frac{k^2}{E_\alpha^*} \, ,
\label{eq:scalar_density} 
\end{align}
%%%%%%%%%%%%%
\begin{align}
\rho_{b3} (r)=\sum_{\alpha=p,n} \left\langle\varphi_\alpha^\dagger(r) \tau_3 \varphi_\alpha(r)\right\rangle
=\rho_{p} (r) - \rho_{n} (r)\, ,
\label{eq:isovect_density}
\end{align}
%%%%%%%%%%%%
\begin{align}
\rho_{s3} (r)=\sum_{\alpha=p,n}  \left\langle\varphi_\alpha^\dagger(r) \tau_3 \beta \varphi_\alpha(r)\right\rangle
=\rho_{sp} (r)-\rho_{sn} (r) \, ,
\label{eq:isoscal_density}
\end{align}
%%%%%%%%%%%%
\begin{align}
\rho_{\rm p}(r)=\sum_\alpha \left\langle\varphi_\alpha^\dagger(r) \left (\frac{1 +\tau_3}{2}
\right) \varphi_\alpha(r)\right\rangle\, ,
\label{eq:charge_density} 
\end{align}
%%%%%%%%%%%%%
\begin{align}
\rho_{\rm T}(r)=\sum_{\alpha=p,n} \left\langle \frac{i}{M} \mbox{\boldmath$\nabla$} \!\cdot\!
\left[ \varphi_\alpha^\dagger(r) \beta \mbox{\boldmath$\alpha$}\varphi_\alpha(r) \right]\right\rangle \, ,
\label{eq:tensor_dens} 
\end{align}
%%%%%%%%%%%
and
%%%%%%%%%%%%%
\begin{align}
\rho_{\rm T,3}(r)=\sum_{\alpha=p,n} \left\langle \frac{i}{M} \mbox{\boldmath$\nabla$} \!\cdot\!
\left[\varphi_\alpha^\dagger(r) \beta \mbox{\boldmath$\alpha$}
\tau_3 \varphi_\alpha(r) \right] \right\rangle \, .  
\label{eq:isotensor_dens} 
\end{align}
%%%%%%%%%%%   
where $E_\alpha^*=\sqrt{k^2+M_\alpha^{*2}}$ is the effective energy density for the nucleons. $M_\alpha^*$ is the effective masses of the nucleons represented as 
%%%%%%%%%%%%%
\begin{align}
M_\alpha^\star=M_\alpha+ \Phi_0 \mp D_0 \, , 
\label{eq:efm_nucleon}
\end{align}
%%%%%%%%%%%
where the $\Phi_0$, $D_0$ are the field equations of $\sigma$, and $\delta$ mesons respectively.

where $g_\sigma$, $g_\omega$, $g_\rho$ and $g_\delta$ are the coupling constants and $m_\sigma$, $m_\omega$, $m_\rho$ and $m_\delta$ are the masses for the $\sigma$, $\omega$, $\rho$ and $\delta$ mesons respectively. $\kappa_3$ (or $\kappa_4$) and $\zeta_0$ are the self-interacting coupling constants of the $\sigma$ and $\omega$ mesons respectively. $\eta_1$, $\eta_2$, $\eta_\rho$ and $\Lambda_\omega$ are the coupling constants of non-linear cross-coupled terms. The quantities $W^{\mu\nu}$ and $\vec R^{\mu\nu}$ being the field strength tensors for the $\omega$ and $\rho$ mesons respectively, defined as $W^{\mu\nu}$ = $\partial^\mu\omega^\nu-\partial^\nu\omega^\mu$ and $\vec R^{\mu\nu}$ = $\partial^\mu\vec\rho^{\,\nu}-\partial^\nu\vec\rho^{\,\mu}$. The $\vec\tau$ are the Pauli matrices and behave as the isospin operator. $M_n$ (= 939 MeV) is the mass of the nucleon. The coupling constants and different meson masses are given in Table \ref{tab:NM_mass_coupling}

In the RMF model, it is assumed that the meson fields are replaced by their expectation values. Also, it is assumed that the system is isotropic in isospin space and the rotationally invariant. The third component of the isospin operator ($\tau_3$) when operates on neutron and proton gives, $\tau_3\ket{p}=(+1)\ket{p}$ and $\tau_3\ket{n}=(-1)\ket{n}$. Applying the relativistic mean-field approximation, the Lagrangian density yields the following Dirac equation for the nucleon field
%%%%%%%%%%%%%%%%
\begin{align}
\Bigg\{i\gamma_{\mu}\partial^{\mu}-g_{\omega}\gamma_{0}\omega-\frac{1}{2}g_{\rho}\gamma_{0}\tau_{3\alpha}\rho-M^\ast_\alpha\Bigg\} \psi_\alpha=0,
\end{align}
%%%%%%%%%%%%%%
where $M^\ast_\alpha$ is the effective mass of the nucleon. Taking into account the third component of the isospin for neutron and proton as defined above, the effective masses of the neutron and proton are given by
%%%%%%%%%%%%%%%%
\begin{align}
M_{p, n}^{\ast}=M_{p,n}-g_{\sigma}\sigma\mp g_{\delta}\delta.
\label{eq:effm_nucleons}
\end{align}
%%%%%%%%%%%%%%
The Lagrangian density can be used to derive  Euler-Lagrange equations of motion for the meson fields with the help of relativistic mean-field approximation as \cite{Sharma_2007, Kumar_2017, Kumar_2018, Kumar_2020}
%%%%%%%%%%%%%%%%
\begin{align}
m_{\sigma}^2\sigma & = g_{\sigma} \sum_{\alpha=p,n}\langle\bar\psi_\alpha\gamma_0\psi_\alpha\rangle - \frac{m_\sigma^2g_\sigma}{M_n}\sigma^2\Bigg(\frac{\kappa_3}{2} + \frac{\kappa_4}{3!}\frac{g_\sigma\sigma}{M_n}\Bigg)
\nonumber\\
&+\frac{g_\sigma}{2M_n}\Bigg(\eta_1 + \eta_2\frac{g_\sigma\sigma}{M_n}\Bigg){ m_\omega^2\omega^2} + \frac{\eta_{\rho}}{2M_n}{g_\sigma}{m_\rho^2 }{\rho^2},
\label{eq:sigma_field}
\end{align}
%%%%%%%%%%%%%%%%
\begin{align}
m_\omega^2\omega & = g_\omega\sum_{\alpha=p,n} \langle\bar\psi_\alpha\psi_\alpha\rangle - \Bigg(\eta_1 + \frac{\eta_2}{2}\frac{g_\sigma\sigma}{M_n}\Bigg)\frac{g_\sigma\sigma}{M_n}m_\omega^2\omega-\frac{1}{3!}\zeta_0g_{\omega}^2\omega^3
\nonumber\\
&- 2\Lambda_{\omega} g_{\omega}^2 g_{\rho}^2 \rho^2 \omega,
\label{eq:omega_field}
\end{align}
%%%%%%%%%%%%%%%%
\begin{align}
m_{\rho}^2 \rho & = \frac{1}{2}g_{\rho} \sum_{\alpha=p,n} \langle\bar\psi_\alpha\tau_3\psi_\alpha\rangle - \eta_\rho \frac{g_\sigma\sigma}{M_n}m_{\rho}^2\rho - 2\Lambda_{\omega} g_\omega^2 g_\rho^2 \omega^2 \rho,
\label{eq:rho_field}
\end{align}
%%%%%%%%%%%%%%%%
\begin{align}
m_\delta^2 \delta & = g_{\delta} \sum_{\alpha=p,n} \langle\bar\psi_\alpha\tau_3\gamma_0\psi_\alpha\rangle. 
\label{eq:delta_field}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Assuming NM as a uniform system, where the fields of $\sigma$, $\omega$ and $\rho$ mesons are independent of position the baryon, scalar, isovector, and isoscalar densities are \cite{Kumar_2018, Kumar_2020}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
n = \sum_{\alpha=p,n} \langle\bar\psi_\alpha\psi_\alpha\rangle  
= n_{p}+n_{n} 
= \sum_{\alpha=p,n}\frac{1}{\pi^2}\int_{0}^{k_{\alpha}} k^2 \, dk,
\label{eq:baryon_density}
\end{align}
%%%%%%%%%%%%%%%%
\begin{align}
n_s = \sum_{\alpha=p,n}\langle\bar\psi_\alpha\gamma_0\psi_\alpha\rangle = n_{sp}+n_{sn} 
= \sum_{\alpha=p,n} \frac{1}{\pi^2}\int_{0}^{k_{\alpha}} k^2 \, dk\, 
\frac{M_{\alpha}^{\ast}} {(k^{2}_{\alpha}+M_{\alpha}^{\ast 2})^{\frac{1}{2}}} ,
\label{eq:scalar_density}
\end{align}
%%%%%%%%%%%%%%%%
\begin{align}
n_3 = \sum_{\alpha=p,n} \langle\bar\psi_\alpha\tau_3\psi_\alpha\rangle = n_p-n_n,
\label{eq:isovector_density}
\end{align}
%%%%%%%%%%%%%%%%
\begin{align}
n_{s3} =\sum_{\alpha=p,n} \langle\bar\psi_\alpha\tau_3\gamma_0\psi_\alpha\rangle = n_{sp}-n_{sn},
\label{eq:isoscalar_density}
\end{align}
%%%%%%%%%%%%%%
where $n_p$ and $n_n$ are the proton and neutron densities respectively, $k_\alpha$ is the nucleon Fermi momentum.

